Optimized Algorithms to Sample Determinantal Point Processes

In this technical report, we discuss several sampling algorithms for Determinantal Point Processes (DPP). DPPs have recently gained a broad interest in the machine learning and statistics literature as random point processes with negative correlation, i.e., ones that can generate a "diverse" sample from a set of items. They are parametrized by a matrix $\mathbf{L}$, called $L$-ensemble, that encodes the correlations between items. The standard sampling algorithm is separated in three phases: 1/~eigendecomposition of $\mathbf{L}$, 2/~an eigenvector sampling phase where $\mathbf{L}$'s eigenvectors are sampled independently via a Bernoulli variable parametrized by their associated eigenvalue, 3/~a Gram-Schmidt-type orthogonalisation procedure of the sampled eigenvectors. In a naive implementation, the computational cost of the third step is on average $\mathcal{O}(N\mu^3)$ where $\mu$ is the average number of samples of the DPP. We give an algorithm which runs in $\mathcal{O}(N\mu^2)$ and is extremely simple to implement. If memory is a constraint, we also describe a dual variant with reduced memory costs. In addition, we discuss implementation details often missing in the literature.

==> manuscript/brouillon.tex <==
One would like to have the coreset guarantee for a minimal number of samples, that is: to find the  marginal probabilities $\pi_i$ minimizing $\mu^*$. 
In order to do so, the first naive approach is to set $\pi_i=\mu\sigma_i/\mathfrak{S}$ such that  $\bar{\pi}_i=\sigma_i/\mathfrak{S}$ for all $i$. This strategy encounters two problems in our setting:
\begin{itemize}
	\item $\bar{\pi}_\text{min}$ may be arbitrarily smaller than $1/N$ (in the general setting,  $\sigma_\text{min}$ may be arbitrarily small) such that $\mu_2^*$ may be arbitrarily large!
	\item $\pi_\text{max}=\mu\sigma_\text{max}/\mathfrak{S}$ may be larger than 1 if $\sigma_\text{max}\geq \mathfrak{S}/\mu$, which is not allowed. 
\end{itemize}
In order to circumvent these difficulties, we will saturate $\bar{\pi}_i$ to a lowest possible value for all $i\in\mathcal{I}_S$ with 
\begin{align}
\mathcal{I}_S = \left\{i ~\text{ s.t. }~ \sigma_i< \frac{1}{N}\right\}
\end{align}
and constrain $\mu$ to be smaller than $\mathfrak{S} / \sigma_\text{max}$. 

\begin{corollary}
	\label{cor:opt_DPP}
	Let us suppose that $\mu \leq \mathfrak{S} / \sigma_\text{max}$. 
	If the marginal probability of inclusion is set to:
	\begin{align}
	\label{eq:pistar1}
	\forall i\in \mathcal{I}_S&\qquad 
	\pi_i^* = \frac{\mu}{N\mathfrak{S}'},\\
	\label{eq:pistar2}
	\forall i \notin\mathcal{I}_S&\qquad
	\pi_i^* = \frac{\mu\sigma_i}{\mathfrak{S}'},
	\end{align}
	with $\mathfrak{S}'$ the normalization constant (such that $\pi^*$ sums to $\mu$)
	\begin{align}
	\mathfrak{S}'=\mathfrak{S} + \sum_{i\in\mathcal{I}_S} \frac{1}{N} - \sigma_i\leq \mathfrak{S} + 1,
	\end{align}
	then, $\mathcal{S}$ is a $\epsilon$-coreset with probability larger than $1-\delta$ provided that:
	\begin{align}
	\label{eq:condition}
	\mu\geq\frac{32\mathfrak{S}'}{\epsilon^2} \left(\epsilon + 4 \mathfrak{S}' \right) \log{\frac{10n}{\delta}}.
	\end{align}
\end{corollary}

\begin{proof}
Suppose that $\pi=\pi^*$ as in Eqs.~\eqref{eq:pistar1}	and~\eqref{eq:pistar2}. The following inequality holds:
\begin{align}
\label{eq:ineq}
\max_i \frac{N\pi_\text{min}^*\sigma_i}{\pi_i^*}\geq 1.
\end{align}
Indeed, if $N\sigma_\text{min}\leq1$, that is, if $\mathcal{I}_S\neq\emptyset$, then $\pi_\text{min}^*=\frac{\mu}{N\mathfrak{S}'}$ and:
\begin{align*}
\max_i \frac{N\pi_\text{min}^*\sigma_i}{\pi_i^*}\geq\max_i\frac{\sigma_i}{\sigma_i} =1.
\end{align*}
Moreover, if $N\sigma_\text{min}> 1$ (\ie, $\mathcal{I}_S=\emptyset$), denote by $j$ the index for which $\pi_i^*$ is minimal and:
\begin{align*}
\max_i \frac{N\pi_\text{min}^*\sigma_i}{\pi_i^*}\geq N\sigma_j \geq N\sigma_\text{min} > 1.
\end{align*}
Inequality~\eqref{eq:ineq} implies that:
\begin{align}
\label{condition:technical}
(\max_i \frac{\sigma_i}{\bar{\pi}_i^*} N\bar{\pi}_\text{min}^*)^2\geq \log{\frac{10}{\delta}}~/~(\log{\frac{10}{\delta}}+\log{n}),
\end{align}
as $n$ is necessarily larger than 1. One can show that Eq.~\eqref{condition:technical} is equivalent to $\mu_1^*\geq \mu_2^*$, such that $\mu^* = \max(\mu_1^*,\mu_2^*)= \mu_1^*$. Replacing $\bar{\pi}_i$ by  $\bar{\pi}_i^*=\pi_i^*/\mu$ in the expression of $\mu_1^*$ yields the result. 
\end{proof}





\begin{remark}
	The constraint $\mu \leq \frac{\mathfrak{S}}{\sigma_\text{max}}$ is often a very loose constraint. We show in the first lemma of Appendix~\ref{app:proof_lemmas} that in the case of $1$-means ($k$-means with $k=1$) and supposing that the data is centered: $\forall i,~ \sigma_i=\frac{1}{N}(1+\frac{\norm{x_i}^2}{v})$, where $v=\frac{1}{N}\sum_x \norm{x}^2$. Thus, $\mathfrak{S}=(N+1)/N$, and the constraint boils down to:
	\begin{align}
	\mu \leq \frac{N+1}{1+\max_i\frac{\norm{x_i}^2}{v}}.
	\end{align}
	Suppose for instance that the underlying distribution is a Gaussian centered in the origin with variance $\nu$. $v$ is the empirical estimator of $\nu$, such that $\max_i\frac{\norm{x_i}^2}{v}$ is the most extreme event of the drawing and is typically smaller than $5$, implying a very loose constraint indeed.
\end{remark}


\begin{remark}
	In many applications (such as in $k$-means detailed in the next section), $N\sigma_\text{min}\geq1$, such that $\mathcal{I}_S=\emptyset$. In this case, $\forall i, ~\pi_i^* = \mu\sigma_i/\mathfrak{S}$, and we recover the classical result that the coreset property is verified provided that
	\begin{align}
	\label{eq:condition_mu}
	\mu\geq\frac{32\mathfrak{S}}{\epsilon^2} \left(\epsilon + 4 \mathfrak{S} \right) \log{\frac{10n}{\delta}}. 
	\end{align}
\end{remark}
